Efficient Algorithms for Bayesian Network Parameter Learning from Incomplete Data

We propose an efficient family of algorithms to learn the parameters of a Bayesian network from incomplete data. In contrast to textbook approaches such as EM and the gradient method, our approach is non-iterative, yields closed form parameter estimates, and eliminates the need for inference in a Bayesian network. Our approach provides consistent parameter estimates for missing data problems that are MCAR, MAR, and in some cases, MNAR. Empirically, our approach is orders of magnitude faster than EM (as our approach requires no inference). Given sufficient data, we learn parameters that can be orders of magnitude more accurate.

==> figs/experiments/alarm2-Mcar-0.3-0.7/overview.tex <==
\begin{tabular}{@{}r|rr|rrrr@{}} \toprule

Size & EM-1 & EM-10 & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline\multicolumn{7}{c}{Runtime [ms]}\\\hline
$10^{2}$ & 483 & 5093 & 3 & 21 & 10 & 17\\
$10^{3}$ & 5993 & 57860 & 20 & 179 & 19 & 100\\
$10^{4}$ & 75781 & 301715 & 192 & 1642 & 172 & 951\\
$10^{5}$ & 309037 & nan & 2466 & 23539 & 3596 & 10077\\
$10^{6}$ & nan & nan & 18843 & 196227 & 19976 & 66679\\
$10^{7}$ & nan & nan & nan & nan & nan & nan\\

\hline\multicolumn{7}{c}{Kullback-Leibler Divergence}\\\hline
$10^{2}$ & 2.2781 & 2.2781 & 2.7148 & 2.4430 & 3.7862 & 3.7822\\
$10^{3}$ & 0.3466 & 0.3463 & 0.5849 & 0.4732 & 0.7416 & 0.7177\\
$10^{4}$ & 0.0445 & nan & 0.1191 & 0.0866 & 0.1775 & 0.1775\\
$10^{5}$ & nan & nan & 0.0159 & 0.0116 & 0.0466 & 0.0530\\
$10^{6}$ & nan & nan & 0.0020 & 0.0014 & 0.0127 & 0.0168\\
$10^{7}$ & nan & nan & nan & nan & nan & nan\\

\hline\multicolumn{7}{c}{Test Set Log-Likelihood (Fully Observed)}\\\hline
$10^{2}$ & -12.047 & -12.047 & -12.442 & -12.173 & -13.542 & -13.538\\
$10^{3}$ & -10.367 & -10.367 & -10.603 & -10.492 & -10.766 & -10.744\\
$10^{4}$ & -10.008 & nan & -10.084 & -10.052 & -10.143 & -10.143\\
$10^{5}$ & nan & nan & -9.978 & -9.973 & -10.008 & -10.015\\
$10^{6}$ & nan & nan & -9.963 & -9.963 & -9.974 & -9.978\\
$10^{7}$ & nan & nan & nan & nan & nan & nan\\

\hline\multicolumn{7}{c}{Training Set Log-Likelihood (Partially Observed)}\\\hline
$10^{2}$ & -9.180 & -9.180 & -9.640 & -9.443 & -10.507 & -10.506\\
$10^{3}$ & -8.798 & -8.798 & -8.946 & -8.876 & -9.100 & -9.093\\
$10^{4}$ & -8.722 & nan & -8.755 & -8.740 & -8.810 & -8.812\\
$10^{5}$ & nan & nan & -8.732 & -8.730 & -8.760 & -8.763\\
$10^{6}$ & nan & nan & -8.728 & -8.728 & -8.738 & -8.740\\
$10^{7}$ & nan & nan & nan & nan & nan & nan\\

\hline\multicolumn{7}{c}{Training Set Log-Likelihood (Fully Observed)}\\\hline
$10^{2}$ & -11.237 & -11.237 & -11.693 & -11.422 & -12.937 & -12.933\\
$10^{3}$ & -10.200 & -10.200 & -10.434 & -10.321 & -10.632 & -10.609\\
$10^{4}$ & -9.980 & nan & -10.051 & -10.018 & -10.114 & -10.114\\
$10^{5}$ & nan & nan & -9.976 & -9.971 & -10.006 & -10.013\\
$10^{6}$ & nan & nan & -9.963 & -9.963 & -9.974 & -9.978\\
$10^{7}$ & nan & nan & nan & nan & nan & nan\\

\bottomrule

\end{tabular}


==> figs/experiments/alarm2-NeighborMar-0.3-2-1.0-0.5/overview.tex <==
\begin{tabular}{@{}r|rr|rrrr@{}} \toprule

Size & EM-1 & EM-10 & F-MCAR & D-MAR & F-MAR & F-MAR\texttt{+}EM\\
\hline\multicolumn{7}{c}{Runtime [ms]}\\\hline
$10^{2}$ & 1110 & 9723 & 11 & 3 & 20 & 756\\
$10^{3}$ & 15341 & 153164 & 71 & 16 & 116 & 12805\\
$10^{4}$ & 153791 & 301143 & 589 & 128 & 830 & 140310\\
$10^{5}$ & 306930 & nan & 11667 & 3082 & 9311 & 307627\\
$10^{6}$ & nan & nan & 70160 & 17578 & 60312 & nan\\
$10^{7}$ & nan & nan & 310862 & 192696 & 331686 & nan\\

\hline\multicolumn{7}{c}{Kullback-Leibler Divergence}\\\hline
$10^{2}$ & 4.4534 & 2.8162 & 4.4791 & 6.1093 & 6.1069 & 2.9383\\
$10^{3}$ & 1.6704 & 0.6611 & 1.6305 & 2.0526 & 2.0384 & 0.6122\\
$10^{4}$ & 1.2883 & nan & 1.0624 & 0.8575 & 0.8557 & 0.1236\\
$10^{5}$ & nan & nan & 0.6508 & 0.3134 & 0.3159 & nan\\
$10^{6}$ & nan & nan & 0.8664 & 0.2238 & 0.2413 & nan\\
$10^{7}$ & nan & nan & nan & 0.1322 & nan & nan\\

\hline\multicolumn{7}{c}{Test Set Log-Likelihood (Fully Observed)}\\\hline
$10^{2}$ & -14.374 & -12.746 & -14.398 & -16.063 & -16.061 & -12.861\\
$10^{3}$ & -11.626 & -10.615 & -11.563 & -11.983 & -11.969 & -10.566\\
$10^{4}$ & -11.241 & nan & -11.018 & -10.811 & -10.809 & -10.079\\
$10^{5}$ & nan & nan & -10.613 & -10.275 & -10.277 & nan\\
$10^{6}$ & nan & nan & -10.829 & -10.186 & -10.203 & nan\\
$10^{7}$ & nan & nan & nan & -10.094 & nan & nan\\

\hline\multicolumn{7}{c}{Training Set Log-Likelihood (Partially Observed)}\\\hline
$10^{2}$ & -9.485 & -9.417 & -10.822 & -12.208 & -12.208 & -9.435\\
$10^{3}$ & -8.839 & -8.791 & -9.642 & -9.912 & -9.904 & -8.791\\
$10^{4}$ & -8.874 & nan & -9.596 & -9.394 & -9.395 & -8.832\\
$10^{5}$ & nan & nan & -9.322 & -8.983 & -8.986 & nan\\
$10^{6}$ & nan & nan & -9.610 & -9.014 & -9.020 & nan\\
$10^{7}$ & nan & nan & nan & -8.891 & nan & nan\\

\hline\multicolumn{7}{c}{Training Set Log-Likelihood (Fully Observed)}\\\hline
$10^{2}$ & -13.527 & -11.888 & -13.582 & -15.358 & -15.357 & -12.031\\
$10^{3}$ & -11.442 & -10.416 & -11.373 & -11.825 & -11.811 & -10.367\\
$10^{4}$ & -11.225 & nan & -11.001 & -10.796 & -10.794 & -10.064\\
$10^{5}$ & nan & nan & -10.611 & -10.274 & -10.276 & nan\\
$10^{6}$ & nan & nan & -10.829 & -10.186 & -10.204 & nan\\
$10^{7}$ & nan & nan & nan & -10.094 & nan & nan\\

\bottomrule

\end{tabular}


==> figs/experiments/fixbb <==
#!/bin/bash

# This is fixbb version 0.31.  Copyright 2000 by Jeff Spirko.
# Redistributable under the GNU General Public License.
# See http://topquark.dhs.org/~spirko/fixbb/

# Changes by Petr Mikulik:
#   -  8.  9. 2000: working file in the $TMP directory; remove backup file
#   - 18. 10. 2000: AWKPARSEBB to support multiple-page (non-EPS) documents
#   - 26. 10. 2000: error if bounding box not determined (GS < 5.50 or empty
#     pages); page status info added

# Options for ghostscript to print the BoundingBox without other junk.
GSOPTS="-dQUIET -dBATCH -dNOPAUSE -sDEVICE=bbox"
export GSOPTS

# Original awk program, checks each line of the file
#AWKPROG='{ if ($1 == "%%BoundingBox:") 
#  print $1, ENVIRON["bbox"]; 
#  else print;}'

# Slightly faster version, doesn't bother looking after finding a BoundingBox.
# What happens if there is more than one BoundingBox?  Can this happen?
AWKPROG='
	(found) { print; next }
	$1 == "%%BoundingBox:" { print $1, ENVIRON["bbox"]; found=1; next }
	{ print }
	'

# Finds min and max of the 4 numbers after the "%%BoundingBox:" label
AWKPARSEBB='
	BEGIN { x1=99999; y1=99999; x2=0; y2=0; page=0 }
	$1!= "%%BoundingBox:" { next }
	$2<0 || $3<0 { next }
	x1>$2 { x1=$2 }
	y1>$3 { y1=$3 }
	x2<$4 { x2=$4 }
	y2<$5 { y2=$5 }
	{ page++; printf "Page " page ": " $0 "  max = " x1 " " y1 " " x2 " " y2  "  \t\r" >"/dev/stderr" }
	END { printf "\t\t\t\t\t\t\t\r" >"/dev/stderr"
	      print x1 " " y1 " " x2 " " y2 }
	'

export bbox

# Each command-line argument is assumed to be a file to process
for FILE in $* ; do

#  BAK=${FILE}~
#  if [ "$TMP" = "" ]; then TMP="."; fi; BAK=$TMP\fixbb__.ps
  BAK='fixbb$$.ps'

  # Get the correct BoundingBox from ghostscript.
  # Old: bbox=`gs ${GSOPTS} ${FILE} 2>&1 | gsort | head -1 | cut -d\  -f 2-`
  bbox=`/usr/bin/gs ${GSOPTS} ${FILE} 2>&1 | awk "$AWKPARSEBB"`

  case $bbox in
    "99999 99999 0 0")
	echo "Bounding box was NOT determined (empty pages or Ghostscript >= 5.50 required)"
	exit ;;
  esac

  echo "Bounding box for \""$FILE"\" is: "$bbox

  # Save the old version of the file
  mv $FILE $BAK

  # Create the new version, replacing the old BoundingBox
  awk "$AWKPROG" $BAK > $FILE

  case `uname` in 
    "OS/2") dos2unix $FILE ;;
  esac

  # delete the backup file
  rm -f $BAK

done


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/90-20-1-1500000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -47.66 & -59.84 & -48.34 & -59.39 & -47.88\\
$10^{3}$ & - & -46.53 & -37.29 & -31.60 & -36.76 & -31.28\\
$10^{4}$ & - & -62.98 & -28.74 & -26.71 & -28.26 & -26.45\\
$10^{5}$ & - & - & -25.88 & -24.97 & -25.43 & -24.75\\
$10^{6}$ & - & - & -25.27 & - & -24.78 & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/90-20-1-300000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -56.23 & -63.34 & -50.55 & -62.38 & -50.06\\
$10^{3}$ & - & -55.04 & -39.89 & -33.34 & -39.09 & -33.01\\
$10^{4}$ & - & -98.20 & -30.46 & -27.26 & -29.73 & -26.98\\
$10^{5}$ & - & - & -28.63 & -26.06 & -27.89 & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/90-20-1-60000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -62.38 & -64.15 & -50.78 & -63.51 & -50.24\\
$10^{3}$ & - & -79.75 & -38.96 & -32.77 & -38.26 & -32.44\\
$10^{4}$ & - & - & -30.65 & -28.61 & -30.05 & -28.34\\
$10^{5}$ & - & - & - & - & - & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/barley-1500000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & -85.11 & -85.53 & -86.00 & -85.74 & -86.24 & -85.80\\
$10^{3}$ & - & -65.96 & -67.88 & -67.23 & -67.79 & -67.15\\
$10^{4}$ & - & -57.21 & -55.34 & -54.56 & -55.05 & -54.43\\
$10^{5}$ & - & - & -51.09 & - & - & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/barley-300000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -85.59 & -85.70 & -85.60 & -85.99 & -85.66\\
$10^{3}$ & - & -67.07 & -67.58 & -66.97 & -67.53 & -66.91\\
$10^{4}$ & - & - & -55.04 & -54.33 & -54.78 & -\\
$10^{5}$ & - & - & - & - & - & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/barley-60000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -85.33 & -85.84 & -85.68 & -86.13 & -85.75\\
$10^{3}$ & - & - & -67.70 & -67.18 & -67.67 & -67.13\\
$10^{4}$ & - & - & -54.93 & - & - & -\\
$10^{5}$ & - & - & - & - & - & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/munin1-1500000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -90.79 & -98.57 & -94.50 & -98.48 & -94.28\\
$10^{3}$ & - & -60.71 & -66.06 & -63.95 & -65.45 & -63.67\\
$10^{4}$ & - & -60.35 & -56.57 & -55.38 & -55.95 & -55.16\\
$10^{5}$ & - & - & -54.29 & -53.38 & -53.67 & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/munin1-300000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -96.51 & -102.51 & -98.21 & -102.40 & -97.95\\
$10^{3}$ & - & -68.04 & -67.82 & -65.49 & -67.21 & -65.22\\
$10^{4}$ & - & -95.01 & -57.68 & -56.00 & -57.05 & -55.79\\
$10^{5}$ & - & - & -54.30 & - & - & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/munin1-60000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -98.95 & -103.59 & -98.68 & -103.54 & -98.49\\
$10^{3}$ & - & -79.83 & -70.49 & -67.27 & -69.78 & -66.97\\
$10^{4}$ & - & - & -59.25 & -57.11 & - & -\\
$10^{5}$ & - & - & - & - & - & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/overview.tex <==
\begin{tabular}{@{}r!{\vrule width 1pt}rr|rr|rr!{\vrule width 1pt}rr|rr|rr@{}} \toprule
Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
 & \multicolumn{6}{c!{\vrule width 1pt}}{90-20-1} & \multicolumn{6}{c}{barley} \\
\hline
$10^{2}$ & - & -62.38 & -64.15 & -50.78 & -63.51 & -50.24 & - & -85.33 & -85.84 & -85.68 & -86.13 & -85.75 \\
$10^{3}$ & - & -79.75 & -38.96 & -32.77 & -38.26 & -32.44 & - & - & -67.70 & -67.18 & -67.67 & -67.13 \\
$10^{4}$ & - & - & -30.65 & -28.61 & -30.05 & -28.34 & - & - & -54.93 & - & - & - \\
$10^{5}$ & - & - & - & - & - & - & - & - & - & - & - & - \\
$10^{6}$ & - & - & - & - & - & - & - & - & - & - & - & - \\
$10^{7}$ & - & - & - & - & - & - & - & - & - & - & - & - \\
\hline
 & \multicolumn{6}{c!{\vrule width 1pt}}{munin1} & \multicolumn{6}{c}{water} \\
\hline
$10^{2}$ & - & -98.95 & -103.59 & -98.68 & -103.54 & -98.49 & - & -19.50 & -20.51 & -19.37 & -20.41 & -19.35 \\
$10^{3}$ & - & -79.83 & -70.49 & -67.27 & -69.78 & -66.97 & - & -16.11 & -16.26 & -15.27 & -16.09 & -15.23 \\
$10^{4}$ & - & - & -59.25 & -57.11 & - & - & - & - & -15.03 & -14.22 & -14.86 & -14.14 \\
$10^{5}$ & - & - & - & - & - & - & - & - & -14.30 & - & - & - \\
$10^{6}$ & - & - & - & - & - & - & - & - & - & - & - & - \\
$10^{7}$ & - & - & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/water-1500000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & -21.30 & -18.66 & -21.58 & -19.87 & -21.36 & -19.83\\
$10^{3}$ & -17.67 & -17.10 & -18.64 & -15.95 & -18.27 & -15.86\\
$10^{4}$ & - & -14.83 & -16.71 & -14.58 & -16.30 & -14.44\\
$10^{5}$ & - & -18.78 & -16.31 & -14.38 & -15.62 & -14.08\\
$10^{6}$ & - & - & -15.25 & - & - & -\\
$10^{7}$ & - & - & -15.13 & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/water-300000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & -18.84 & -18.06 & -21.23 & -19.61 & -21.07 & -19.57\\
$10^{3}$ & - & -14.99 & -16.47 & -15.33 & -16.24 & -15.26\\
$10^{4}$ & - & -17.39 & -15.59 & -14.52 & -15.26 & -14.43\\
$10^{5}$ & - & - & -15.22 & - & - & -\\
$10^{6}$ & - & - & -15.09 & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.3-2-1.0-0.5/water-60000/overview.tex <==
\begin{tabular}{@{}r|rr|rr|rr@{}} \toprule

Size & EM-JT & EM-BP & D-MCAR & F-MCAR & D-MAR & F-MAR\\
\hline
$10^{2}$ & - & -19.50 & -20.51 & -19.37 & -20.41 & -19.35\\
$10^{3}$ & - & -16.11 & -16.26 & -15.27 & -16.09 & -15.23\\
$10^{4}$ & - & - & -15.03 & -14.22 & -14.86 & -14.14\\
$10^{5}$ & - & - & -14.30 & - & - & -\\
$10^{6}$ & - & - & - & - & - & -\\
$10^{7}$ & - & - & - & - & - & -\\

\bottomrule

\end{tabular}


==> overview/BP-NIPS/NeighborMar-0.9-2-0.5-0.5/overview.tex <==
\begin{table*}
\centering
\input{\detokenize{./90-20-1-1500000/overview.tex}}
\caption{\detokenize{90-20-1-1500000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./90-20-1-300000/overview.tex}}
\caption{\detokenize{90-20-1-300000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./90-20-1-60000/overview.tex}}
\caption{\detokenize{90-20-1-60000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./barley-1500000/overview.tex}}
\caption{\detokenize{barley-1500000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./barley-300000/overview.tex}}
\caption{\detokenize{barley-300000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./barley-60000/overview.tex}}
\caption{\detokenize{barley-60000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./munin1-1500000/overview.tex}}
\caption{\detokenize{munin1-1500000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./munin1-300000/overview.tex}}
\caption{\detokenize{munin1-300000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./munin1-60000/overview.tex}}
\caption{\detokenize{munin1-60000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./water-1500000/overview.tex}}
\caption{\detokenize{water-1500000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./water-300000/overview.tex}}
\caption{\detokenize{water-300000}}
\end{table*}

\begin{table*}
\centering
\input{\detokenize{./water-60000/overview.tex}}
\caption{\detokenize{water-60000}}
\end{table*}


